Meta-SAGE: Scale Meta-Learning Scheduled Adaptation with Guided Exploration for Mitigating Scale Shift on Combinatorial Optimization

This paper proposes Meta-SAGE, a novel approach for improving the scalability of deep reinforcement learning models for combinatorial optimization (CO) tasks. Our method adapts pre-trained models to larger-scale problems in test time by suggesting two components: a scale meta-learner (SML) and scheduled adaptation with guided exploration (SAGE). First, SML transforms the context embedding for subsequent adaptation of SAGE based on scale information. Then, SAGE adjusts the model parameters dedicated to the context embedding for a specific instance. SAGE introduces locality bias, which encourages selecting nearby locations to determine the next location. The locality bias gradually decays as the model is adapted to the target instance. Results show that Meta-SAGE outperforms previous adaptation methods and significantly improves scalability in representative CO tasks. Our source code is available at https://github.com/kaist-silab/meta-sage

==> sections/03_2_meta_learning.tex <==
\section{Training \ours{}}
\label{sec:learning}
This section provides a formulation of \ours{} and a meta-learning scheme for SML. We provide a pseudo-code in \cref{append:training_algo}. 


\subsection{Bi-level Formulation of Training \ours{}} \label{sec:SML}

The role of \meta{} is to give appropriately transformed embedding to the subsequent parameter adaptation (i.e., \adpt{}) based on the scale information.
We formulate our training of \ours{} as a bi-level optimization problem as follows:

% (Training SML)
\begin{align}
    \label{eq:upper_opt}
    \max_{\textcolor{darkgreen}{\phi}} \quad  &  \mathbb{E}_{P(\bm{x})} \mathbb{E}_{p_{\theta^*, \phi, \textcolor{darkblue}{\eta}}} \left[ R (\bm{a}_{1:N}, \bm{x}) \right]  \\
    \label{eq:lower_opt}
    \mbox{s.t.} \quad  & \textcolor{darkblue}{\eta} \leftarrow \text{\adpt{}}(\bm{x}, K; \theta^{*}, \textcolor{darkgreen}{\phi})
\end{align}

The upper-level optimization (i.e., training SML) in \cref{eq:upper_opt} contains $\eta$ that can be obtained by solving the lower-level optimization (i.e., SAGE). At the same time, the lower-level requires optimized $\phi$ as an input. Therefore, the optimization problems are inter-related, which makes the training unstable.

\subsection{Meta learning with Distillation Scheme}

We decompose the bi-level optimization by simulating SAGE operator without $\phi$ and training SML to amortize the pre-simulated results.
In other words, \meta{} learns the transformation to the $K$ adapted embedding using the scale information.

\textbf{Distillation objective.} 

Directly Learning the results of SAGE operation with more than one-shot can lead overfitting to a specific problem $\boldsymbol{x}$.
Model-agnostic meta-learning \citep[MAML; ][]{finn2017model} can be the solution for overfitting, but it requires complex computation and is sometimes unstable \citep{antoniou2019train}. 
We suggest a simple but effective meta-learning objective using a distillation scheme. 

The objective is defined as imitating the results of simulated $\eta^*$ as follows:

\begin{equation}
    \mathcal{J}_{\text{distil}} (\phi) = -\frac{1}{L}\sum_{l=1}^{L}\|g_{\phi}(\boldsymbol{h}_{(l)},N_{(l)}) - g_{\eta^{*}_{(l)}}(\boldsymbol{h}_{(l)} )\|_2,
\end{equation}

where $\eta^{*}_{(l)}$ is obtained by simulating $\text{\adpt{}}(\bm{x}_{(l)}, K; \theta^*)$ for each instance $\{ \bm{x}_{(l)} \}_{l=1}^{L} \sim P(\bm{x}|N)P(N)$, and $\bm{h}_{(l)}$ is obtained by the encoder with pre-trained parameter $\theta^*$.

By reducing the differences $g_\phi(\cdot)$ and , the parameter $\phi$ is uniformly distilled by $\eta^{*}_{(1)},\ldots,\eta^{*}_{(L)}$, the $\phi$ is expected to be located at the sweet spot similar to the MAML.

\textbf{Zero-shot simulation objective. } To improve the effectiveness of SML, we include zero-shot simulation objective to the final objective function.
The scale-wise transformed context embedding can be directly plugged into \adpt{}, which means the $g_\phi(\bm{h}, N)$ works as SAGE operation with $K=0$.
Therefore, \meta{} needs to be trained to maximize the \adpt{} objective function in \cref{eq:j_sage} with the policy $p_{\theta^*}(\cdot|\bm{x}, N, \phi)$ instead of $p_{\theta^*}(\cdot|\bm{x},\eta)$.
The zero-shot simulation objective function is defined with the shared parameter $\phi$ over the problem distribution $P(\bm{x}|N)P(N)$ as follows:
\begin{equation*}
    \mathcal{J}_{\text{sim}}(\phi) = \mathbb{E}_{\bm{x} \sim P(\bm{x}|N)P(N)}\left[\mathcal{J}_{\text{SAGE}}(\phi;\bm{x}) \right].
\end{equation*}
The SAGE objective function $\mathcal{J}_{\text{SAGE}}$ is contextualized by $\bm{x}$. By taking expectation over the problem distribution, the shared parameter $\phi$ is trained over the problem distribution $P(\bm{x}|N)P(N)$.

Finally, we get the SML objective function as follows:
\begin{equation*}
    \mathcal{J}_{\text{SML}}(\phi) = \mathcal{J}_{\text{distil}}(\phi) + \beta \mathcal{J}_{\text{sim}}(\phi),
\end{equation*}
where $\beta$ is a tunnable hyperparameter.

==> tables/ablation1.tex <==
\centering
\caption{{Ablation study for SAGE components. Locality and Temp. stand for locality bias SoftMax temperature, respectively. }}\label{abl:sage}
\scalebox{0.9}{
\begin{tabular}{ccccc}
\toprule[1.0pt]
\multicolumn{2}{c}{Scheduling} &  \multicolumn{2}{c}{Tasks}\\
\cmidrule(lr{0.2em}){1-2}\cmidrule(lr{0.2em}){3-4}
Locality& Temp. & TSP & CVRP \\
\midrule

  & & 18.63&63.98\\
\checkmark  & & 18.36&63.91 \\
 & \checkmark  &17.73 & 63.25\\
\checkmark  & \checkmark & \textbf{17.56}&\textbf{63.17} \\
\bottomrule[1.0pt]
\end{tabular}
}






